RoAST: Robustifying Language Models via Adversarial Perturbation with Selective Training

Fine-tuning pre-trained language models (LMs) has become the de facto standard in many NLP tasks. Nevertheless, fine-tuned LMs are still prone to robustness issues, such as adversarial robustness and model calibration. Several perspectives of robustness for LMs have been studied independently, but lacking a unified consideration in multiple perspectives. In this paper, we propose Robustifying LMs via Adversarial perturbation with Selective Training (RoAST), a simple yet effective fine-tuning technique to enhance the multi-perspective robustness of LMs in a unified way. RoAST effectively incorporates two important sources for the model robustness, robustness on the perturbed inputs and generalizable knowledge in pre-trained LMs. To be specific, RoAST introduces adversarial perturbation during fine-tuning while the model parameters are selectively updated upon their relative importance to minimize unnecessary deviation. Under a unified evaluation of fine-tuned LMs by incorporating four representative perspectives of model robustness, we demonstrate the effectiveness of RoAST compared to state-of-the-art fine-tuning methods on six different types of LMs, which indicates its usefulness in practice.

==> Figures/Fig_ablation.tex <==
\begin{figure*}[t]
\begin{center}
    {
    \subfigure[Effect of $\lambda$]
        {
        \includegraphics[width=0.315\textwidth]{Figures/files/consistency.pdf}
        \label{fig:fig3a}
        }
    \subfigure[Effect of $\alpha$]
        {
        \includegraphics[width=0.315\textwidth]{Figures/files/sparsity.pdf}
        \label{fig:fig3b}
        } 
    \subfigure[Effect of $\beta$]
        {
        \includegraphics[width=0.315\textwidth]{Figures/files/smoothness.pdf}
        \label{fig:fig3c}
        }
    }
\end{center}
\caption{Comparison of robustness from \name{} under different hyper-parameter choices. \textbf{[Not Fixed]}}
\label{fig:fig_abl}
\end{figure*}

==> Tables/NLP_analysis.tex <==
\begin{table*}[ht]
    \caption{Robustness of fine-tuned RoBERTa-large with \name{} under different masking strategies. All the values are mean across 3 random seeds and results with variance are presented in Appendix \ref{supp_more}.}
    \vspace{-0.1in}
    \begin{center}
    \begin{adjustbox}{width=.96\linewidth}
	\begin{tabular}{r|ccccca|ccccca}
		\toprule
		\multicolumn{1}{c}{} & \multicolumn{6}{c}{Entailment} & \multicolumn{6}{c}{Sentiment Classification} \\
		Method & Acc$_{\tt in}$ & Acc$_{\tt shift}$ & Acc$_{\tt adv}$ & ECE ($\downarrow$) & AUROC & $\Delta_{\tt avg}$ & Acc$_{\tt in}$ & Acc$_{\tt shift}$ & Acc$_{\tt adv}$ & ECE ($\downarrow$) & AUROC & $\Delta_{\tt avg}$ \\ \midrule
		Vanilla & 89.97 & 64.31 & 48.60 & 12.64 & 92.09 & 0.00 & 96.29 & 91.79 & 66.30 & 7.11 & 86.72 & 0.00 \\
		Min & 90.68 & 64.37 & 50.87 & 11.89 & 90.89 & 0.44 & 96.22 & 91.97 & 71.45 & 5.61 & 86.70 & 7.26 \\
		Rand & 90.65 & 64.13 & 50.98 & 11.39 & 91.13 & 1.67 & 96.22 & 92.25 & 72.68 & 5.19 & 90.03 & 14.88\\
		\name{} & {90.64} & {63.95} & 51.33 & 11.02 & {93.25} & {7.63} & {96.87} & {92.38} & {72.57} & {5.45} & {90.37} & {18.39} \\
		\bottomrule
	\end{tabular}
    \end{adjustbox}
    \end{center}
    \vspace{-0.1in}
    \label{table:nlp_diff_policy}
\end{table*}


==> our_mask_policy.tex <==
\begin{algorithm}[t!]
   \caption{Sampling Gradient Mask from Relative Importance Scores}
   \label{alg:mask}
\begin{algorithmic}
  \State
  \textbf{Input:} Relative importance scores $\{s(\theta)|\theta \in \Theta \}$, masking ratio $\alpha$, smoothness factor $\beta$ 
  \For{each parameter $\theta \in \Theta$}
  \State $\widetilde{s}(\theta)\leftarrow \text{argsort}(s(\theta)) / |\{\theta\}| $ ~ {\color{Gray2} // Normalization with relative order} 
  \State $p(\theta) \leftarrow 1 / (1 + \text{exp}(2\beta(\widetilde{s}(\theta)-\alpha))) $ ~ {\color{Gray2} // Smooth approximation of thresholding} 
  \State $m(\theta) \sim \text{Bernoulli}\big(p(\theta)\big)$ ~ {\color{Gray2} // Sampling mask from Bernoulli distribution} 
  \EndFor 
  \State \textbf{Return: $\{m(\theta)|\theta \in \Theta\}$}
\end{algorithmic}
\end{algorithm}

